An Unsupervised Approach towards Varying Human Skin Tone Using Generative Adversarial Networks

With the increasing popularity of augmented and virtual reality, retailers are now focusing more towards customer satisfaction to increase the amount of sales. Although augmented reality is not a new concept but it has gained much needed attention over the past few years. Our present work is targeted towards this direction which may be used to enhance user experience in various virtual and augmented reality based applications. We propose a model to change skin tone of a person. Given any input image of a person or a group of persons with some value indicating the desired change of skin color towards fairness or darkness, this method can change the skin tone of the persons in the image. This is an unsupervised method and also unconstrained in terms of pose, illumination, number of persons in the image etc. The goal of this work is to reduce the time and effort which is generally required for changing the skin tone using existing applications (e.g., Photoshop) by professionals or novice. To establish the efficacy of this method we have compared our result with that of some popular photo editor and also with the result of some existing benchmark method related to human attribute manipulation. Rigorous experiments on different datasets show the effectiveness of this method in terms of synthesizing perceptually convincing outputs.

==> bibliography.tex <==
@manual{image_source0,
title  = "",
author = "",
note="\url{https://p4t6u7k5.stackpathcdn.com/wp-content/uploads/shutterstock_605616227.jpg}"
}
@manual{image_source1,
title  = "",
author = "",
note="\url{https://i1.wp.com/cbtpsychology.com/wp-content/uploads/2018/10/Therapy.jpg}"
}

@manual{image_source2,
title  = "",
author = "",
note="\url{https://designpanoply.com/blog/how-to-change-a-persons-skin-color-from-dark-to-light-in-photoshop}"
}
@manual{video_source2,
title  = "",
author = "",
note="\url{https://www.youtube.com/watch?v=pO7gq_2BvZw}"
}

@manual{wikiAR,
title  = "",
author = "",
note="\url{https://en.wikipedia.org/wiki/Augmented_reality}"
}
@manual{newsMIT,
title  = "",
author = "",
note="\url{https://www.technologyreview.com/2019/10/23/238473/augmented-reality-in-retail-virtual-try-before-you-buy/}"
}
@manual{link3,
titlMISCe  = "",
author = "",
note="\url{https://retailwire.com/discussion/}"
}
% will-augmented-reality-tech-effectively-bring-the-try-on-experience-online/
@inproceedings{pix2pix,
  title={Image-to-image translation with conditional adversarial networks},
  author={Isola, Phillip and Zhu, Jun-Yan and Zhou, Tinghui and Efros, Alexei A},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1125--1134},
  year={2017}
}
@article{lgvton,
  title={LGVTON: A Landmark Guided Approach to Virtual Try-On},
  author={Roy, Debapriya and Santra, Sanchayan and Chanda, Bhabatosh},
  journal={arXiv preprint arXiv:2004.00562},
  year={2020}
}
@misc{kstest,
  title={Roy, Handbook of Methods of Applied Statistics, 1 (1967)},
  author={Chakravarti, Laha},
  publisher={John Wiley and Sons}
}
@article{ssim,
  title={Image quality assessment: from error visibility to structural similarity},
  author={Wang, Zhou and Bovik, Alan C and Sheikh, Hamid R and Simoncelli, Eero P and others},
  journal={IEEE transactions on image processing},
  volume={13},
  number={4},
  pages={600--612},
  year={2004}
}
@article{naji2019survey,
  title={A survey on skin detection in colored images},
  author={Naji, Sinan and Jalab, Hamid A and Kareem, Sameem A},
  journal={Artificial Intelligence Review},
  volume={52},
  number={2},
  pages={1041--1087},
  year={2019},
  publisher={Springer}
}
@article{kakumanu2007survey,
	title={A survey of skin-color modeling and detection methods},
	author={Kakumanu, Praveen and Makrogiannis, Sokratis and Bourbakis, Nikolaos},
	journal={Pattern recognition},
	volume={40},
	number={3},
	pages={1106--1122},
	year={2007},
	publisher={Elsevier}
}

@article{shaik2015comparative,
	title={Comparative study of skin color detection and segmentation in HSV and YCbCr color space},
	author={Shaik, Khamar Basha and Ganesan, P and Kalist, V and Sathish, BS and Jenitha, J Merlin Mary},
	journal={Procedia Computer Science},
	volume={57},
	number={12},
	pages={41--48},
	year={2015},
	publisher={Elsevier}
}

@inproceedings{kanzawa2011human,
	title={Human skin detection by visible and near-infrared imaging},
	author={Kanzawa, Yusuke and Kimura, Yoshikatsu and Naito, Takashi},
	booktitle={IAPR Conference on Machine Vision Applications},
	volume={12},
	pages={14--22},
	year={2011},
	organization={Citeseer}
}


@inproceedings{nunez2008detection,
	title={Detection of human skin in near infrared hyperspectral imagery},
	author={Nunez, Abel S and Mendenhall, Michael J},
	booktitle={IGARSS 2008-2008 IEEE International Geoscience and Remote Sensing Symposium},
	volume={2},
	pages={II--621},
	year={2008},
	organization={IEEE}
}


@article{al2015hybrid,
	title={Hybrid human skin detection using neural network and K-means clustering technique},
	author={Al-Mohair, Hani K and Saleh, Junita Mohamad and Suandi, Shahrel Azmin},
	journal={Applied Soft Computing},
	volume={33},
	pages={337--347},
	year={2015},
	publisher={Elsevier}
}

@article{zuo2017combining,
	title={Combining convolutional and recurrent neural networks for human skin detection},
	author={Zuo, Haiqiang and Fan, Heng and Blasch, Erik and Ling, Haibin},
	journal={IEEE Signal Processing Letters},
	volume={24},
	number={3},
	pages={289--293},
	year={2017},
	publisher={IEEE}
}

@article{tan2011fusion,
	title={A fusion approach for efficient human skin detection},
	author={Tan, Wei Ren and Chan, Chee Seng and Yogarajah, Pratheepan and Condell, Joan},
	journal={IEEE Transactions on Industrial Informatics},
	volume={8},
	number={1},
	pages={138--147},
	year={2011},
	publisher={IEEE}
}


@inproceedings{brand2000comparative,
	title={A comparative assessment of three approaches to pixel-level human skin-detection},
	author={Brand, Jason and Mason, John S},
	booktitle={Proceedings 15th International Conference on Pattern Recognition. ICPR-2000},
	volume={1},
	pages={1056--1059},
	year={2000},
	organization={IEEE}
}


@article{kolkur2017human,
	title={Human skin detection using RGB, HSV and YCbCr color models},
	author={Kolkur, Seema and Kalbande, D and Shimpi, P and Bapat, C and Jatakia, Janvi},
	journal={arXiv preprint arXiv:1708.02694},
	year={2017}
}


@article{nguyen2018new,
	title={A new efficient approach to detect skin in color image using Bayesian classifier and connected component algorithm},
	author={Nguyen-Trang, Thao},
	journal={Mathematical Problems in Engineering},
	volume={2018},
	year={2018},
	publisher={Hindawi}
}

@inproceedings{shen2017learning,
	title={Learning residual images for face attribute manipulation},
	author={Shen, Wei and Liu, Rujie},
	booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
	pages={4030--4038},
	year={2017}
}


@inproceedings{wang2018weakly,
	title={Weakly supervised facial attribute manipulation via deep adversarial network},
	author={Wang, Yilin and Wang, Suhang and Qi, Guojun and Tang, Jiliang and Li, Baoxin},
	booktitle={2018 IEEE Winter Conference on Applications of Computer Vision (WACV)},
	pages={112--121},
	year={2018},
	organization={IEEE}
}
@inproceedings{scfegan,
  title={SC-FEGAN: Face Editing Generative Adversarial Network with User's Sketch and Color},
  author={Jo, Youngjoo and Park, Jongyoul},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={1745--1753},
  year={2019}
}

@article{he2019attgan,
	title={Attgan: Facial attribute editing by only changing what you want},
	author={He, Zhenliang and Zuo, Wangmeng and Kan, Meina and Shan, Shiguang and Chen, Xilin},
	journal={IEEE Transactions on Image Processing},
	volume={28},
	number={11},
	pages={5464--5478},
	year={2019},
	publisher={IEEE}
}


@inproceedings{zhang2018sparsely,
	title={Sparsely grouped multi-task generative adversarial networks for facial attribute manipulation},
	author={Zhang, Jichao and Shu, Yezhi and Xu, Songhua and Cao, Gongze and Zhong, Fan and Liu, Meng and Qin, Xueying},
	booktitle={Proceedings of the 26th ACM international conference on Multimedia},
	pages={392--401},
	year={2018}
}

@inproceedings{chen2009automatic,
	title={Automatic skin color beautification},
	author={Chen, Chih-Wei and Huang, Da-Yuan and Fuh, Chiou-Shann},
	booktitle={International Conference on Arts and Technology},
	pages={157--164},
	year={2009},
	organization={Springer}
}
@inproceedings{is,
title={Improved techniques for training gans},
author={Salimans, Tim and Goodfellow, Ian and Zaremba, Wojciech and Cheung, Vicki and Radford, Alec and Chen, Xi},
booktitle={Advances in neural information processing systems},
pages={2234--2242},
year={2016}
}
@inproceedings{fid,
title={Gans trained by a two time-scale update rule converge to a local nash equilibrium},
author={Heusel, Martin and Ramsauer, Hubert and Unterthiner, Thomas and Nessler, Bernhard and Hochreiter, Sepp},
booktitle={Advances in Neural Information Processing Systems},
pages={6626--6637},
year={2017}
}
@inproceedings{deepfashion,
title={Deepfashion: Powering robust clothes recognition and retrieval with rich annotations},
author={Liu, Ziwei and Luo, Ping and Qiu, Shi and Wang, Xiaogang and Tang, Xiaoou},
booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
pages={1096--1104},
year={2016}
}
@inproceedings{hourglass,
  title={Stacked hourglass networks for human pose estimation},
  author={Newell, Alejandro and Yang, Kaiyu and Deng, Jia},
  booktitle={European conference on computer vision},
  pages={483--499},
  year={2016},
  organization={Springer}
}
@inproceedings{lipssl,
  title={Look into person: Self-supervised structure-sensitive learning and a new benchmark for human parsing},
  author={Gong, Ke and Liang, Xiaodan and Zhang, Dongyu and Shen, Xiaohui and Lin, Liang},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={932--940},
  year={2017}
}
@inproceedings{perceptual_loss,
  title={Perceptual losses for real-time style transfer and super-resolution},
  author={Johnson, Justin and Alahi, Alexandre and Fei-Fei, Li},
  booktitle={European conference on computer vision},
  pages={694--711},
  year={2016},
  organization={Springer}
}

@inproceedings{multiposevton,
title={Towards multi-pose guided virtual try-on network},
author={Dong, Haoye and Liang, Xiaodan and Shen, Xiaohui and Wang, Bochao and Lai, Hanjiang and Zhu, Jia and Hu, Zhiting and Yin, Jian},
booktitle={Proceedings of the IEEE International Conference on Computer Vision},
pages={9026--9035},
year={2019}
}
@article{cgan,
title={Conditional generative adversarial nets},
author={Mirza, Mehdi and Osindero, Simon},
journal={arXiv preprint arXiv:1411.1784},
year={2014}
}
@inproceedings{imagenet,
AUTHOR = {Deng, J. and Dong, W. and Socher, R. and Li, L.-J. and Li, K. and Fei-Fei, L.},
TITLE = {{ImageNet: A Large-Scale Hierarchical Image Database}},
BOOKTITLE = {CVPR09},
YEAR = {2009},
BIBSOURCE = "http://www.image-net.org/papers/imagenet_cvpr09.bib"} 

@inproceedings{gan,
title={Generative adversarial nets},
author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle={Advances in neural information processing systems},
pages={2672--2680},
year={2014}
}

@inproceedings{ms-ssim,
  title={Multiscale structural similarity for image quality assessment},
  author={Wang, Zhou and Simoncelli, Eero P and Bovik, Alan C},
  booktitle={The Thrity-Seventh Asilomar Conference on Signals, Systems \& Computers, 2003},
  volume={2},
  pages={1398--1402},
  year={2003},
  organization={Ieee}
}
@inproceedings{inceptionv3,
title={Rethinking the inception architecture for computer vision},
author={Szegedy, Christian and Vanhoucke, Vincent and Ioffe, Sergey and Shlens, Jon and Wojna, Zbigniew},
booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
pages={2818--2826},
year={2016}
}

